Logarithmic Regret for Adversarial Online Control

We introduce a new algorithm for online linear-quadratic control in a known system subject to adversarial disturbances. Existing regret bounds for this setting scale as $\sqrt{T}$ unless strong stochastic assumptions are imposed on the disturbance process. We give the first algorithm with logarithmic regret for arbitrary adversarial disturbance sequences, provided the state and control costs are given by known quadratic functions. Our algorithm and analysis use a characterization for the optimal offline control law to reduce the online control problem to (delayed) online learning with approximate advantage functions. Compared to previous techniques, our approach does not need to control movement costs for the iterates, leading to logarithmic regret.

==> section_stationary.tex <==
%!TEX root = paper.tex
\newcommand{\ftil}{\widetilde{f}}
\newcommand{\xalg}{x^{\Alg}}
\newcommand{\ualg}{u^{\Alg}}

This section highlights the technical challenges encountered when attempting to apply \olws{} to attain logarithmic regret in online control with adversarial disturbances. In addition to highlighting the advantages (no pun intended) of our \olwax approach, we hope this appendix also serves an an informal tutorial of prior approaches for online control problems. The section is organized as follows:
\begin{enumerate}
	\item \pref{app:olws_overview} gives an intuitive overview of the \olws{} paradigm, explaining that the regret encountered by the learner incurs a `stationarization' cost reflecting the mismatch between the costs induced by the learner's actual visited trajectory, and the trajectories considered by the stationary costs.
	\item \pref{app:advantage over OLws} explains that the dominant approach for bounding stationarization cost is in terms of a ``movement cost'', which measures the cumulative differences between succesive policies $\pi_t$: informally, $\sum_{t=1}^T\|\pi_t - \pi_{t-1}\|$. Pointing forward to \pref{app:exp_concave_perils}, we explain that this is the major impediment to attain logarithmic regret in our setting. In contrast,  stationarization/movement costs \emph{do not} arise in our analysis of \olwa{}, making this new approach preferable for our setting.
	\item \pref{app:olws_for_online_control} explains in greater detail how the \olwsx paradigm has been applied to online control with adversarial disturbances. \pref{app:oco_memory} explains the OCO-with-memory framework due to \cite{anava2015online}. \pref{app:movement_costs_online_control} explain how \cite{agarwal2019online} instantiate this framework for online control with the \dap{} parametrization, detailing that the (approximate) stationary costs functions $f_{t;h}(M)$ that arise, and the corresponding movement cost in the regret analysis. Examining these loss functions from \cite{agarwal2019online}, \pref{app:stat_cost_exp_conc_nut_strong_convex} explains that the (approximate) stationary $f_{t;h}(M)$ are exp-concave but not strongly convex.
	\item  \pref{app:exp_concave_perils} demonstrates that, in the OCO-with-memory framework, the the movement cost for  sequencess of exp-concave but non-strongly convex functions can scale as $\bigoh(\sqrt{T})$ in the worst case. This implies that any analysis which uses a black-box reduction to OCO-with-memory with bounded movement cost cannot guarantee rates faster that $\bigoh(\sqrt{T})$.\footnote{Note that this argument does not preclude the possibility that the \olws{} algorithms can attain logarithmic regret; rather, it demonstrates the an analysis which passes through movement costs for arbitrary exp-concave stationary costs are insufficient.}
\end{enumerate}
Finally, \pref{app:mdpe} compares our \olwax approach to the \mdpex algorithm proposed by \cite{even2009online}. These two algorithms are superficially similiar, because they both consider  control-theoretic advantages. Despite these similarities, we note that \mdpex is still an instance of \olws, and therefore succumbs to the limitations described above. In addition, we explain that the analysis of \mdpex is ill-suited to settings with adversarial dynamics, such as the one considered in this work.


\subsection{Overview of OLwS}
\label{app:olws_overview}
In this section, we give an overview of the online learning with stationary costs ($\olwsx$) framework for online control and discuss some challenges associated with using it to attain logarithmic regret for online linear control. In \olws, one defines the stationary costs
\begin{align}
\lambda_t(\pi;\matw) := \ell(x_t^{\pi}(\matw),u_t^{\pi}(\matw)),\label{eq:lookback}
\end{align}
which is the cost suffered that would be suffered at time $t$ had the policy $\pi$ had used at all previous rounds \citep{yadkori2013online,anava2015online,agarwal2019online,simchowitz2020improper}.\footnote{Many works also consider ``steady state'' costs obtained by taking $t \to \infty$ for a given policy \citep{even2009online,abbasi2014tracking,cohen2018online,agarwal2019logarithmic}, but this formulation is ill-posed in our setting due to the adversarial dynamics.} By construction, $\lambda_t(\pi;\matw)$ does not depend on the state of the system. Moreover, if $\pi$ is an executable policy (i.e., $\pi_t(x;\matw)$ depends only on $x$ and $w_{1:t-1}$), then $\lambda_t(\pi;\matw)$ can be determined exactly at time $t$. At each round $t$, $\olws$ selects a policy $\pi^{(t)}$ to minimize regret on the sequence $\lambda_t(\pi;\matw)$, and follows $u_t = \pi_t^{(t)}(x;\matw)$. The total regret is decomposed as
\begin{align}
\Reg(\pialg;\matw,\Pi) =  \Big(\underbrace{\sum_{t=1}^T \ell(x_t^{\Alg}, u_t^{\Alg})-  \lambda_t(\pi^{(t)};\matw) }_{\text{(stationarization cost)}} \Big) +   \Big(\underbrace{\sum_{t=1}^T \lambda_t(\pi^{(t)};\matw)-  \inf_{\pi \in \Pi} \sum_{t=1}^T  \lambda_t(\pi;\matw)}_{(\lambda\text{-regret})} \Big). \label{eq:lookback_reg}
\end{align}
To our knowledge, all known applications of \olwsx bound the stationarization cost via the movement cost in \pref{eq:movement_cost}. 

\subsection{Avoiding Stationarization Cost: Our advantage over OLwS. \label{app:advantage over OLws}} \olwsx optimizes stationary costs $\lambda_t(\pi)$, which correspond to the loss suffered by the adversary at round $t$ if policy $\pi$ had been students at each time $t$. To relate the stationary costs to the learner's cost, the \olwsx proposes the bounding the following movement cost:
\begin{align}
\text{movement cost } := \sum_{t}\|\pi^{(t)} - \pi^{(t-1)}\|, \quad \text{(informal)}, \label{eq:movement_cost}
\end{align}
When the movement costs are small, the learner's state at time $t$, $x^\Alg_t$, is similar to the states that would be obtained by selecting $\pi^{(t)}$ at all time $s < t$, namely $x^{\pi}_t$. \pref{app:olws_limits} explains how the cost \pref{eq:movement_cost} arises  in more detail.
%
While standard online learning algorithm ensure $\sqrt{T}$-movement cost, online gradient descent (\ogd) shows that if $\lambda_t$ is strongly convex (in a suitable parametrization), the movement cost is $\log T$ \citep{anava2015online}. Since \ogdx also ensures logarithmic regret on the $\lambda_t$-sequence, the combined algorithm ensures logarithmic regret overal.

The natural stationary costs that arise in our problem are ``exp-concave'' \citep{hazan2011newtron}, an intermediate between the two regimes. Exp-concave functions $\lambda_t$ are strongly convex in the local geometry induced by $(\nabla \lambda_t)(\nabla \lambda_t)^\top $, but not necessarily in other directions. This is sufficient for logarithmic regret, but as we explain in \pref{app:exp_concave_perils}, known methods cannot leverage this property to ensure logarithmic bounds on the relevant movement cost. 
%
Here in lies the advantage (no pun intended) of $\olwa$: by considering the \emph{future} costs of an action (by way of the advantage-proxy $\advhat$) rather than the stationary costs, we avoid the technical challenge of bounding the movement cost in the elusive exp-concave regime.

% \subsection{Policy Regret and Online Convex Optimization with Memory \label{app:oco_memory}}
\subsection{Applying \olws{} to online control \label{app:olws_for_online_control}}
\subsubsection{Policy regret and online convex optimization with memory \label{app:oco_memory}}
A useful instantiation of the \olws{} paradigm is the policy-regret setting introduced by  \cite{arora2012online}, which considers stationary costs with finite memory.  This work considers online learning with loss functions $f_t(z_t,\dots,,z_{t-h})$, and defines policy regret for the iterate sequence $\{z_t\}_{t=1}^{T}$ as $\sum_{t}f(z_{t},\dots,z_{t-h}) - \inf_z \sum_{t}f_t(z,\dots,z)$. Algorithms for this setting work with a  \emph{unary} loss $\widetilde{f}_t(z) = z \mapsto f_t(z,\dots,z)$,which can be viewed as a special case of the stationary cost $\lambda_t$ defined above where $z \in \cC$ encodes a policy and $f_t(z,\dots,z)$ is the loss suffered if $z$ had been selected throughout the game. \cite{arora2012online} take this approach in an expert setting and \cite{anava2015online} consider a setting where $\ftil$ is an arbitrary convex loss, which they call \emph{Online Convex Optimization with Memory}. In this setting, the stationarization cost arises via the decomosition
\begin{align}
\text{(policy regret)} =  \Big(\underbrace{\sum_{t=1}^T f_t(z_t,\dots,z_{t-h}) - \ftil_t(z_t) }_{\text{(stationarization cost)}} \Big) +   \Big(\underbrace{\sum_{t=1}^T \ftil_t(z_t) -  \inf_{z \in \cC} \sum_{t=1}^T  \ftil_t(z)}_{(\lambda\text{-regret})} \Big). \label{eq:lookback_reg_policy}
\end{align}
As we explain in the sequel, for stable linear systems, one can approximate the full stationary costs $\lambda_t$ via costs $\ftil_t$ with finite memory. When $f_t$ are Lipschitz in all arguments, \cite{anava2015online} bound the stationarization cost in terms of movement cost in terms of. They show
\begin{align*}
\sum_{t=1}^T f_t(z_t,\dots,z_{t-h}) - \ftil_t(z_t)  \le \sum_{t=1}^T |f_t(z_t,\dots,z_{t-h}) - \ftil_t(z_t)| \le \bigoh\prn*{h^2 L}\sum_{t=1}^T \|z_t - z_{t-1}\|,
\end{align*}
where $L$ is an appropriate Lipschitz constant. Note that this inequality formalizes \pref{eq:movement_cost} for this setting.


\cite{anava2015online} demonstrated that many popular online convex optimization algorithms naturally produce slow-moving iterates, leading to policy regret bounds in \pref{eq:lookback_reg_policy}. In particular, they show that applying online gradient descent on the unary losses leads to $\poly(h) \cdot \sqrt{T}$-policy regret when $\widetilde{f}_t$ are convex and Lipschitz, and $\frac{\poly(h)}{\alpha} \cdot \log T$-policy regret when $\widetilde{f}_t$ are $\alpha$-strongly convex. Notably, \cite{anava2015online} do not show that logarithmic regret is attainable for the more general family of exp-concave losses, which are more natural for the setting in this paper.

\subsubsection{ OCO with memory for Online Control\label{app:movement_costs_online_control}}
Let us presently consider the online linear control settting, illustrating that the relevant movement cost which arrises is in terms of the $M_t$ matrices. Following \cite{agarwal2019online}, we apply OCO with memory to our setting using the \dapx parametrization (\pref{def:dap}), where $\pi^{(t)}$ is given by $\pi^{(M_t)}$, for a matrix $M \in \cM_0 = \cM(m,R,\gamma)$ selected at time $t$.  


\cite{agarwal2019online} show stationary costs $\lambda_t$ in \pref{eq:lookback} can be approximated up to
arbitrarily accuracy by functions $\ftil_{t;h}(M)$, which depend only on the most recent $m+h$ disturbances $w_{t-(m+h):t}$, and where $h = \mathrm{poly}(\log T, \frac{1}{1-\gamma})$. They also show that the suffered loss $\loss(\xalg_t,\ualg_t)$ can be approximate via $f_{t;h}(M_{t-h:t})$, which also depends on recent disturbances, and which specializes to $\widetilde{f}_{t:h}(M)$ when $M_{t-h:t} = (M,\dots,M)$. Precisely, for $M \in \cM$, define the inputs.
\begin{align*}
u_{s}(M;\matw) = \sum_{i=1}^m M^{[i]} w_{s-i}
\end{align*}
Then, the functions $f_{t:h}(M_{t:t-h})$ and $\widetilde{f}_{t:h}(M)$ takes the form
\begin{align}
f_{t;h}(M_{t-h:t}) &:= \loss\prn*{\alpha_t(\matw) + \sum_{i=1}^m \Psi_i u_{t-i}(M_{t-i};\matw), u_{t}(M_t;\matw)- \Kinf \sum_{i=1}^m \Psi_i u_{t-i}(M_{t-i};\matw) }, \nonumber
\\
\ftil_{t;h}(M) &:=\loss\prn*{\alpha_t(\matw) + \sum_{i=1}^m \Psi_i u_{t-i}(M;\matw), u_{t}(M;\matw)- \Kinf \sum_{i=1}^m \Psi_i u_{t-i}(M;\matw) },\label{eq:stat_control_cost}
\end{align}
where functions $\alpha_t(\matw)$ is a function $w_{1:t}$ and $A,B$ but \emph{not} on the learners inputs, and $\Psi_i = (A+B\Kinf)^{i-1}B$.


With this parameterization, the regret decomposition for OCO with memory takes the form
\begin{align}
\dapReg(\pialg;\matw) =  \Big(\underbrace{\sum_{t=1}^T f_{t;h}(M_{t-h:t})  - \ftil_{t;h}(M_t) }_{\text{(stationarization cost)}} \Big) +
\Big(\underbrace{\sum_{t=1}^T \ftil_{t;h}(M_t)-  \inf_{\pi \in \Mst} \sum_{t=1}^T  \ftil_{t;h}(M)}_{(\lambda\text{-regret})} \Big) + \bigoht\prn*{1}. \label{eq:lookback_reg_dap}
\end{align}
% Note that we perform online learning online on the $\ftil_{t;h}$ sequence, and bound the stationarization costs only in the analysis. 
In this setting $f_{t;h}(\cdot)$ is Lipschitz so---following arguments from \cite{anava2015online}---we have
\begin{align*}
\text{(stationarization cost)} \le h^2 \poly(m,R,(1-\gamma)^{-1})\cdot \sum_{t=1}^T \|M_{t} - M_{t-1}\|_{\mathrm{F}},
\end{align*}
where the right-hand side is a movement cost for the iterates (formalizing \pref{eq:movement_cost}), and where we recall $h$ is the memory horizon, where $m,R,\gamma$ are the parameters defining the set of \dap{} controllers $\cM_0$, and where we consider Frobenius norm movement $\|M_{t} - M_{t-1}\|_{\mathrm{F}} = \sqrt{\sum_{i \ge 0}\|M_{t}^{[i]} - M_{t-1}^{[i]}\|_{\mathrm{F}}^2}$ (which induces the standard Euclidean geometry considered in gradient descent). 

In general, the bound on the movement cost will depend on the choice of regret minimization algorithm. Many natural algorithms ensure bounds on the movement cost which are on the same order as their bounds on regret. For example, exponential weights and online gradient descent ensure $\sqrt{T}$-bounds \citep{even2009online,yu2009markov,anava2015online}, and for strongly convex losses, FTPL and online gradient descent ensure logarithmic movement \citep{abbasi2014tracking,anava2015online}.

\subsubsection{The Stationary Costs for \dap{} are Exp-Concave but not Strongly Convex\label{app:stat_cost_exp_conc_nut_strong_convex}}
For the \dapx parametrization, the functions that naturally arise are exp-concave, but not necessarily strongly convex. To see this, consider the loss $\loss(x,u) = \|x\|^2 + \|u\|^2$. We obseve that the stationary costs considered by \cite{agarwal2019online}, made explicit in \pref{eq:stat_control_cost}, are the sum of two quadratic functions of the form considered in \pref{lem:exp_concave_quadratic}, and are thus exp-concave.
\footnote{The sum of two $\alpha$-exp-concave functions is $\frac{\alpha}{2}$-exp-concave. For a proof, observe that $(\nabla (f+g))^\top (\nabla (f+g))^\top \preceq 2(\nabla f)(\nabla f)^\top  + 2(\nabla g)(\nabla g)^\top$. Hence, if $f$ and $g$ are $\alpha$-exp concave, we have $\nabla^2 (f+g) \succeq \alpha (\nabla f)(\nabla f)^\top  + \alpha(\nabla g)(\nabla g)^{\top}\succeq \frac{\alpha}{2}(\nabla (f+g))^\top (\nabla (f+g))^\top$.} However, $\ftil_{t;h}(M)$ is \emph{not} strongly convex in general.  For example, if the noise sequence is \emph{constant}, say $w_t = w_{t-1} = \dots = w_1$, then $\nabla u_t(M;\matw)$ is identical for all $t$ and thus $\nabla^2 \widetilde{f}_{t;h}(M)$ is a rank one matrix.

% \subsection{The perils of exp-concave movement costs\label{app:exp_concave_perils}}
\subsection{Movement costs in general exp-concave online learning\label{app:exp_concave_perils}}
In this section, we explain the challenge of achieving low-movement cost in the OCO-with-memory with framework, which elucidates the broader challenge of relating stationary costs to regret in \olwsx. We give an informal sketch for an exp-concave OCO-with-memory setting in which the online Newton step algorithm (\pref{alg:ons}) fails to achieve logarithmic regret. Consider a simple class of functions with scalar domain and length-$1$ memory:
\begin{align*}
f_t(z_1,z_2) = (1 - (w_t z_1 + w_{t-1}z_2))^2, \quad \ftil_t(z) = f_t(z,z),
\end{align*}
where $(w_{t})$ are parameters chosen by the adversary.
We use the constraint set $z \in \cC:= [-1/5,1/5]$%, so that $\max_{z \in \C} (1 - (w_t z_1 + w_{t-1}z_2))^2$ \dfcomment{max: what was this supposed to be?}. 
Policy regret (paralleling \pref{eq:lookback_reg_dap}) is given by
\begin{align*}
\text{(policy regret)} &= \sum_{t=1}^T f_t(z_t,z_{t-1}) - \inf_{z} \sum_{t=1}^T \ftil_t(z) \\
&= \underbrace{\left(\sum_{t=1}^T f_t(z_t,z_{t-1}) - \ftil_t(z_t) \right)}_{\text{(stationarization cost)}}  + \underbrace{\left(\sum_{t=1}^T \ftil_t(z_t)   - \inf_{z} \sum_{t=1}^T \ftil_t(z) \right)}_{\text{(}\lambda-\text{regret)}}.
\end{align*}
We now construct a sequence of loss functions where the $\lambda$-regret for \ons{} is logarithmic, but where standard upper bounds on stationary cost can grow as $\Omega(\sqrt{T})$. Consider the sequence $w_t = (-1)^t + \frac{\mu}{2}$, where $\mu = 1/\sqrt{T}$. We see that $\ftil_t(z) = (1 - \mu z)^2$. We remark that this function is only $\mu^2 = 1/T$-strongly convex, so that the guarantees for strongly convex online gradient descent are vacuous \cite{hazan2016introduction}, necessitating the use of \ons.

Let us see what happens if we try to leverage exp-concavity. From \pref{lem:exp_concave_quadratic}, $\ftil_t(z)$ are $\frac{1}{4}$-exp-concave on the set $\cC$. Hence, if we run \ons{} (\pref{alg:ons}) with an appropriate learning rate, $\lambda$-regret scales logarithmically \citep{hazan2016introduction}:
\begin{align*}
\sum_{t=1}^T \ftil_t(z_t) - \min_{z \in \cC} \sum_{t=1}^T \ftil_t(z) \le \bigoh\prn*{\log T}.
\end{align*}
Let us now turn to the stationarization cost, $\sum_{t=1}^T f_t(z_t,z_{t-1}) - \ftil_{t}(z_t)$. The approach of \cite{anava2015online}, is to bound the per-step errors, $|f_t(z_t,z_{t-1}) - \ftil_{t}(z_t)|$. We can directly see that 
\begin{align*}
f_t(z_t,z_{t-1}) - \ftil_{t}(z_t) &= (1 - w_t z_t - w_{t-1}z_t)^2 - (1 - w_t z_t - w_{t-1}z_{t-1})^2\\
&= -2w_{t-1}(1 - w_t z_t)^\top (z_t - z_{t-1}) + w_{t-1}^2(z_{t-1}+z_{t})(z_{t}-z_{t-1})^2\\
&= (-2w_{t-1}(1 - w_t z_t)^\top + w_{t-1}^2(z_{t-1}+z_{t})) (z_t - z_{t-1}).
\end{align*}
For $\mu$ sufficiently small and $z \in \cC$, we can check that $|(-2w_{t-1}(1 - w_t z_t)^\top + w_{t-1}^2(z_{t-1}+z_{t}))| \ge \frac{1}{16}$, so that
\begin{align*}
|f_t(z_t,z_{t-1}) - \ftil_{t}(z_t)| \ge \frac{|z_t - z_{t-1}|}{16}.
\end{align*}
Thus, we have
\begin{align*}
\sum_{t=1}^T |f_t(z_t,z_{t-1}) - \ftil_{t}(z_t)| \ge \frac{1}{16}\cdot \text{(movement cost)}, \quad \text{ where }\quad\text{(movement cost)} = \frac{1}{6}\sum_{t=1}^T|z_{t}-z_{t-1}|.
\end{align*}
We now show that this movement cost is large. For simplicity, we keep our discussion informal to avoid navigating the projection step in \ons. Without projections, we have
\begin{align*}
|z_t - z_{t-1}| = \left|\epsilon + \sum_{s=1}^{t-1} \nabla^2 \ftil_s(z_s)\right|^{-1}(\nabla \ftil_{t-1}(z_{t-1})).
\end{align*}
Observe that for each $z \in \cC$, $\nabla^2 \ftil_s(z) = \mu^2 = 1/T$, so that  we have $\epsilon + \sum_{s=1}^{t-1} \nabla^2 \ftil_s(z_s) = (1+\epsilon)$. On the other hand, for $z \in \cC$, we can lower bound $|\nabla \ftil_{t-1}(z)| \ge \frac{\mu}{2}  = \frac{1}{2\sqrt{T}}$. Hence, 
\begin{align*}
\text{(movement cost)} = \frac{1}{16}\sum_{t=1}^T|z_{t}-z_{t-1}| \ge \frac{\sqrt{T}}{32(1+\epsilon)}.
\end{align*}
Here, we note that the standard implementation perscribes $\epsilon$ to be constant, giving us $\Omega(\sqrt{T})$ movement. Moreover, increasing $\epsilon$ will degrade the corresponding regret bound, preventing logarithmic combined regret.
Note that increasing $\epsilon$ to $1/T^{1/4}$ will partially mitigate the movement cost, but at the expense of increasing the regret on the $\ftil_t$ sequence.



\subsection{Comparison with MDP-E \label{app:mdpe}}%\label{sssec:compare_to_MDPE}}
\mdpex \citep{even2009online} is an instantiation of \olwsx for MDPs with known non-adversarial dynamics and time varying adversarial losses $\loss_t$. In this setting the stationary costs $\lambda_t(\pi)$ represent the long-term costs of a policy $\pi$ under the loss $\loss_t$ (if one prefers, the loss can be treated as fixed, and $w_t$ can encode loss information). To achieve low regret on the $\lambda_t$-sequence, \mdpex maintains policy iterates $\{\pi^{(t)}_x\}$ for all states $x$, and selects its action according to the policy for the corresponding current state: \[u_t^{\Alg} \gets \pi^{(t)}_{x^{\mathrm{alg}}_t}(x_t^{\Alg}).\] The policy sequence $\pi^{(t)}_x$ is selected to minimize regret on a certain $Q$-function: $\lambda_{t,x}(\pi) : \pi \mapsto Q^{\pi}(x,\pi(x))$ (here, policies and Q-functions are regarded as stationary). Under the assumption that the dynamics under benchmark policies are also stationary, achieving low regret on each $\{\lambda_{t,x}\}$-sequence simultaneously for all $x$ ensures low $\lambda$-regret (in the sense of Eq.\eqref{eq:lookback_reg}) over the trajectory $x_t^\Alg$.\footnote{See the proof of \citet[Theorem 5]{even2009online}, which uses that the induced state distribution is does not change with $t$.} 
As a consequence, \mdpex is ill-suited to settings with adversarially changing dynamics. Since \olwax considers Q-functions and advantages defined with respect to an \emph{fixed} policy $\pistar$, it does not require benchmark policies to have stationary dynamics (which is important, since our adversarial disturbance setting does not have stationary dynamics).

Moreover, like the stationary costs $\lambda_{t,x}(\pi)$ also describe long-run performance under $\pi$, and still need to be related to the learner's realized trajectory, typically via a bound on the movement cost of the policies. As described above, the analysis of \olwax does not require bounding the movement cost.


\begin{comment}


\subsection{\olwsx with Exp-Concavity Losses}

As we explain in Appendix [], for a fixed quadratic loss, the stationary costs that arises (or rather, close approximations thereof) are exp-concavity functions of the $\widetilde{f}_{t;h}(M;\matw) = \sum_{z \in \{x,u\}}\|A_{z,t} \mathrm{vec}(M)  - b_{z,t}\|_{\Sigma_{z,t}}^2$, where $\mathrm{vec}(M)$ denotes the m



\paragraph{\olwsx in online control.}



 For the simple loss $\loss(x,u)$, the function $\widetilde{f}_{t;h}(M;\matw)$ can be rendered as 

For simplicity, consider the strongly convex $\loss(x,u) = \|x\|^2 + \|u\|^2$.
 Even if for such an $\ell$, we see that $\widetilde{f}_{t;h}(M)$ is \emph{not} strongly convex.  Nevertheless, $\widetilde{f}_{t;h}(M;\matw)$ have a special, quadratic form: for $z \in \{x,u\}$, there exists rank-deficient and time-varying linear operators $\cL_{t,h;z}(M;\matw)$ and $M$-independent $q_{t,h;z}(\matw)$ such that $\widetilde{f}_{t;h}(M;\matw) = \sum_{z \in \{x,u\}}\|\cL_{t,h;z}(M;\matw) -   q_{t,h;z}(\matw)\|_{2}^2$. By \pref{lem:quadratic_exp_concave}, functions of this form satisfy the exp-concavity guarantee (\pref{def:exp_concave}), a local 




\begin{lemma}
\end{lemma}
\begin{proof} Consider a scalar system $(A,B)$, where $B = 1$, with $A = \rho + \kappa$, and controllered by stabilizing controller $\kappa$, and with $m = 1$. Note then that $(A-BK) = \rho$. From \citep{agarwal2019online}, the function takes the form 
\begin{align*}
f_{t;h}(M_{t},\dots,M_{t-h}) = (x_{t;h}^{M_{t-h:t}}(w_{t-h:t}))^2 + \frac{R}{\kappa^2} (u_{t;h}^{M_{t:-h:t}}(w_{t-h:t}))^2
\end{align*}
where $x_{t;h}^{M_{t-h:t}}(\matw) = \sum_{s=t-h}^{t} (A-B\kappa)^{t-s} w_s + \sum_{s=t-h}^{t-1} (A-B\Kinf)^{t-s-1} B M_{s}w_{s}$, and $u_{t;h}^{M_{t:-h:t}}(w_{t-h:t}) =  - \kappa x_{t;h}^{M_{t-h:t}}(\matw) + M_s$. For the special case of $B = 1$, and $\rho = (A - B\kappa)$, $x_{t;h}^{M_{t-h:t}}(w_{t-h:t}) = \sum_{s=t-h}^{t} \rho^{t-s} w_s + \sum_{s=t-h}^{t-1} \rho^{t-s-1} w_{s} M_s$. In particular, if $\|w_s - 1\| \le \epsilon$ for all $t$ and $\rho = 1/2$, then for $M_{s} = M$ for $t \in [h]$, we have 
\newcommand{\Err}{\mathrm{Err}}
\begin{align*}
x_{t;h}^{M}(w_{t-h:t}) = 2 + 2 M + \Err_{t,h;x}(M),
\end{align*}
where $\Err_h(M) = \dots$. 
\begin{align*}
u_{t;h}^{M}(w_{t-h:t}) = M -\kappa(2+2M)+ \Err_{t,h;u}(M),
\end{align*}
Hence,
\begin{align*}
\loss(x) &= 4(1 + M)^2 + \frac{1}{\kappa^2}(M -2\kappa(1+M)) \Err_{h}(M) \\
&= 4\left((1+M)^2 + (\frac{-M}{2\kappa} + (1+M))\right)^2 +\Err_{h}(M)
\end{align*}

Let $A = \begin{bmatrix} 0 & 1 &1 \\ 0 & 0 & 0 \\
0& 0 & 0 \end{bmatrix}$. Then $A^2 = \begin{bmatrix} 0 & 1 & 0 \\ 0 & 0 & 0 \\
0& 0 & 0 \end{bmatrix}$, and $A^3 = 0$. Moreover, let $B = \begin{bmatrix} 0 \\ 1 \\ 0 \end{bmatrix}$. Then, $A$

, and finally suppose that $w_t = z_t e_1$, in the $e_1$ direction. Then, we have that
\begin{align*}
x^M_t = e_1 \left(w_t + B M w_{t-1})  \right)
\end{align*}

\begin{align*}
f_{t;h}(M_{t},\dots,M_{t-h}) &= \Ru (-\kappa x_{t;h}^{M_{t-h:t}}(\matw) +  M_t w_{t})^2 + \kappa^2 x_{t;h}^{M_{t-h:t}}(\matw)^2\\
&= (1+\Ru\kappa^2)(x_{t;h}^{M_{t-h:t}}(\matw)^2) + 
 (-\kappa x_{t;h}^{M_{t-h:t}}(\matw) +  M_t w_{t})^2 + \kappa^2 
\end{align*}




Thus, with $\Kinf = 1$,
\begin{align*}
-u_{t;h}^{M_{t-h:t}}(\matw) = x_{t;h}^{M_{t-h:t}}(\matw) - \sum_{i=1}^m  w_{t - i} M_{s}^{[i]}
\end{align*}
\end{proof}



When $\dimx = \dimu = 1$, $m = 1$, and $\loss(x,u) = x^2 + u^2$, then $f_{t;h}$ has the form
\begin{align*}
f_{t;h}(M_{t},\dots,M_{t-h}) = (\alpha_{t;x} + \sum_{i=1}^h \beta_{t,i;x} M_{t-i} )^2 + (\alpha_{t;u} + \sum_{0=1}^h \beta_{t,i;u} M_{t-i} )^2
\end{align*}
for appropriate, time varying $\alpha_{t;x},\beta_{t,s;x}$ and $\alpha_{t;u},\beta_{t,s;u}$.









For the $\dap$ parametrize policies $\pi^{(M)}$ \pref{def:dap}, one can approximate the stationary costs by costs which only look bad $h$ steps: 
\begin{align*}
\lambda_{t;h}(\pi^{(M)};\matw) &= \loss(x_{t;h}^{M}(\matw) , -\Kinf x_{t;h}^M(\matw) + \sum_{i=1}^{m} \Psi_s M^{[i]}w_{s-m}),
\end{align*}
where, defining $\Psi_s = (A-B\Kinf)^{s-1}B$, $= x_{t}^{\Kinf}(\matw) + \sum_{s=t-h}^{t-1}\sum_{i=1}^{m} \Psi_s M^{[i]}w_{s-m}$ is the state that would arise if additional inputs where added at time steps $t-h,\dots,t$.


where , and $x_{t}^{\Kinf}(\matw)$ are the sequence that arise if the feedback law $\Kinf$ was used without additional input \cite{agarwal2019online}\footnote{\cite{agarwal2019online} also truncate $u_{t}^{\Kinf}(\matw),x_{t}^{\Kinf}(\matw)$ as well, but this does not change the functional form of the dependence on $M$.} The finite lookback follows from the fact that the underlying system $A+B\Kinf$ is stable. By the same token, one can approximate $\loss(\xalg_t,\ualg_t) \approx \overline{\lambda}_{t;h}[\pi^{(M)}_{t},\dots,\pi^{(M)}_{t-h};\matw]$, where
\begin{align*}
\overline{\lambda}_{t;h}[\pi^{(M_t)},\dots,\pi^{(M_{t-h})};\matw] = \loss( x_{t}^{\Kinf}(\matw) + \sum_{s=t-h}^{t-1}\sum_{i=1}^{m} \Psi_s M_{s}^{[i]}w_{s-m} , u_{t}^{\Kinf}(\matw) + \sum_{i=1}^{m} M_t^{[i]}w_{t-m}),
\end{align*}


%\label{sssec:compare_to_olws}}
Let us now compare \olwax to the \olwsx approach for adressing state-dependence. We begin by expositing an abstract online RL setting, where $\matw$ encodes the influence of the adversary (e.g. on the loss or dynamics), and $\pi$ are arbitrary policies suitably parametrized. 
,  We note that in episodic settings , the stationary costs exactly capture the regret \citep{zimin2013online}.


Here, the stationarization cost captures the discrepancy between the loss suffered at time $t$ on at state $x_t^{\Alg}$ that arose from playing $u_s = \pi^{(s)}_s(x;\matw)$ at each $s < t$, versus the loss suffered at time $t$ that \emph{would} have according if the algorithm played according to $\pi^{(t)}$ at each rounds; a penalty \cite{anava2015online} deems ``the price of past mistakes''. Under common mixing and Lipschitz-loss assumptions, the stationarization cost is bounded by the \emph{movement cost}, which informally measures the magnitude of the change in iterates, in an appropriate norm $\|\cdot\|$. Specifically, if the loss $\ell$ are $L$-Lipschitz in both arguments, one 



\subsection{\olwsx in online control}




\subsection{Online Convex Optimization with Memory}
We now describe how \dap's yield a convex control parametrization, and how this translates into a a bound on $\dapReg$.  While discussion focuses on the control setting of \cite{agarwal2019online}, we our expositions captures the essential elements of a broad range of work online RL, including tabular MDPs and tracking. We refer this approach loosely as online convex optimization with memory (\ocom), although there are a few minor differences between our exposition and prior formulations \citep{anava2015online,agarwal2019online}; we expound upon these in Appendix []. 

Consider the \emph{stationary} cost function which describes the cost at time $t$ if the policy $\pim$ can be selected at each round $s \le t$; formally:
\begin{align*}
\lambda_t(M;\matw) := \ell(x_t^{\pim}(\matw),u_t^{\pim}(\matw)).
\end{align*}
One can verify that $M \mapsto (x_t^{\pi^{M}}(\matw),u_t^{\pi^{M}}(\matw))$ is an \emph{affine} function, rendering $\lambda_t(M;\matw) $ convex. With this observation, \cite{agarwal2019online} propose using the online-convex optimization with memory strategy of \cite{anava2015online}: at each round, use an online convex optimization algorithm to produced iterates $M_t$ in such a way as to minimize what we term the $\statreg$:
\begin{align*}
(\statreg)\ldef\quad \sum_{t=1}^T \lambda_t(M_t;\matw) - \inf_{M \in \cM}\sum_{t=1}^T\lambda_t(M;\matw)
\end{align*}
For this sequence of interates $M_t$, they propose the policy $\pi^{\Alg}$ defined by $\pi^{\Alg}_t(x) = \pi^{(M_t)}(x)$ (we note that the iterates $M_t$ themselves depend on prior states and $w_s$'s).  Since $\lambda_t(\cdot;\matw)$ is convex, standard online learners can achieve $O(\sqrt{T})$ $\statreg$. Moreover, if $\ell(\cdot,\cdot)$ is \emph{quadratic}, then second-order online learners can achieve $\statreg$ that scales as $\log T$. 

Unfortunately, $\statreg$ differs from the $\dapReg$ by a ``stationarization cost'', which reflects the mismatch between the iterates $x_t^{\pi^{\Alg}}$ produced by the algorithm, and the stationarized iterates $x_t^{\pi^{(M_t)}}$ considered by the stationary cost. Indeed, using $\sum_{t=1}^T\lambda_t(M;\matw) = \cost(\pim)$, and suppressing $\matw$-dependence for simplicity, we have
\begin{align}
\dapReg(\pi;\matw,\cM) &= \cost(\pi^{\Alg}) - \sum_{t=1}^T \lambda_t(M_t;\matw) + (\statreg)\nonumber\\
&= \underbrace{\sum_{t=1}^T \ell(x_t^{\Alg},u_t^{\Alg}) -  \ell(x_t^{\pi^{(M_t)}},u_t^{\pi^{(M_t)}})}_{(\text{stationarization cost})}  + (\statreg). \label{eq:stat_reg_decomp}
\end{align}
Therefore, even if $\statreg = \bigoh(\log T)$, the $\statcost$ might be considerably larger. In Section [], we explain the standard methods approach for bounding $\statcost$ in terms of the iterate ``movement cost'', and highglight challenges of ensuring sub-$\sqrt{T}$ $\statcost$ in our present setting. 


\paragraph{The online learning with memory reduction.} To our knowledge, every existing (non-episodic) online control and RL algorithm adopt  the following ``online learning wiht memory'' reduction ($\olwm$), which we describe informally. At time $t$, $\olwm$ strategies run a low-regret online learner on ``idealized'' losses $f_t(\pi_t)$ which capture the cost at time $t$ if policy $\pi_t$ had been selected for all time steps $t,t-1,\dots,$. The low-regret online learner then ensures that $\sum_{t}f_t(\pi_t) - \min_{\pi \in \Pi} \sum_{t=1}^T f_t(\pi)$ is small. Of course, the learners ``actual loss'' at time $t$ is a function $F_t[\pi_t,\pi_{t-1},\dots]$ which depends on all past policy policies; and thus the actual policy regret is instead 
\begin{align}
\sum_{t=1}^T F_t[\pi_t,\pi_{t-1},\dots] -  \min_{\pi \in \Pi} \sum_{t=1}^T f_t(\pi)\label{eq:pol_reg}.
\end{align}
We note that the comparator term \emph{is} in terms of the idealized loss $f_t(\pi)$, since the benchmark assumes $\pi$ was selected for all steps of the game. 


To establish that the regret in Eq.~\eqref{eq:pol_reg} is small, these analyses  argue that the sum actual losses $\sum_t F_t[\pi_t,\pi_{t-1},\dots]$ are well-approximated by their idealizations $\sum_t f_t(\pi_t)$. This requires two steps. First, one argues that the system \emph{mixes}, or has limited memory. Thus, $F_t[\pi_t,\pi_{t-1},\dots]$ can be well approximated by a function $\widetilde{F}_{t}[\pi_t,\dots,\pi_{t-h}]$ which only depends on recent policies. Second, one argues that policies $\pi_t$ procedured the online learner are \emph{slow-moving}, in that $\pi_t \approx \pi_{t-1}$. For small $h$, this ensures that $\widetilde{F}_{t}[\pi_t,\pi_{t-1},\dots,\pi_{t-h}] \approx \widetilde{F}_{t}[\pi_t,\pi_t,\dots,\pi_{t}] \approx f_t(\pi_t)$, recovering the idealized loss.  


\paragraph{Beyond online learning with memory.} In many environments, the mixing assumption is quite natural (in linear control, for example, policies 
which do not mix may incur arbitrarily large costs). However, as we show in this paper, the slow moving condition can be quite restrictive in attaining fast rates for onlie control problems. 
\end{comment}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

